Do Large Language Models Solve the Problems of Agent-Based Modeling? A Critical Review of Generative Social Simulations

Recent advancements in AI have reinvigorated Agent-Based Models (ABMs), as the integration of Large Language Models (LLMs) has led to the emergence of ``generative ABMs'' as a novel approach to simulating social systems. While ABMs offer means to bridge micro-level interactions with macro-level patterns, they have long faced criticisms from social scientists, pointing to e.g., lack of realism, computational complexity, and challenges of calibrating and validating against empirical data. This paper reviews the generative ABM literature to assess how this new approach adequately addresses these long-standing criticisms. Our findings show that studies show limited awareness of historical debates. Validation remains poorly addressed, with many studies relying solely on subjective assessments of model `believability', and even the most rigorous validation failing to adequately evidence operational validity. We argue that there are reasons to believe that LLMs will exacerbate rather than resolve the long-standing challenges of ABMs. The black-box nature of LLMs moreover limit their usefulness for disentangling complex emergent causal mechanisms. While generative ABMs are still in a stage of early experimentation, these findings question of whether and how the field can transition to the type of rigorous modeling needed to contribute to social scientific theory.

==> tables/RQ1.tex <==
\begingroup
    \renewcommand*{\arraystretch}{1.5}%
    \definecolor{tabred}{RGB}{230,36,0}%
    \definecolor{tabgreen}{RGB}{0,116,21}%
    \definecolor{taborange}{RGB}{255,124,0}%
    \definecolor{tabbrown}{RGB}{171,70,0}%
    \definecolor{tabyellow}{RGB}{255,253,169}%
    \newcommand*{\redtriangle}{\textcolor{tabred}{\ding{115}}}%
    \newcommand*{\greenbullet}{\textcolor{tabgreen}{\ding{108}}}%
    \newcommand*{\orangecirc}{\textcolor{taborange}{\ding{109}}}%
    \newcommand*{\headformat}[1]{{\small#1}}%
    \newcommand*{\vcorr}{%
      \vadjust{\vspace{-\dp\csname @arstrutbox\endcsname}}%
      \global\let\vcorr\relax
    }%
    \newcommand*{\HeadAux}[1]{%
      \multicolumn{1}{@{}r@{}}{%
        \vcorr
        \sbox0{\headformat{\strut #1}}%
        \sbox2{\headformat{Complex Data Movement}}%
        \sbox4{\kern\tabcolsep\redtriangle\kern\tabcolsep}%
        \sbox6{\rotatebox{45}{\rule{0pt}{\dimexpr\ht0+\dp0\relax}}}%
        \sbox0{\raisebox{.5\dimexpr\dp0-\ht0\relax}[0pt][0pt]{\unhcopy0}}%
        \kern.75\wd4 %
        \rlap{%
          \raisebox{.25\wd4}{\rotatebox{45}{\unhcopy0}}%
        }%
        \kern.25\wd4 %
        \ifx\HeadLine Y%
          \dimen0=\dimexpr\wd2+.5\wd4\relax
          \rlap{\rotatebox{45}{\hbox{\vrule width 4cm height .4pt}}}%
        \fi
      }%
    }%
    \newcommand*{\head}[1]{\HeadAux{\global\let\HeadLine=Y#1}}%
    \newcommand*{\headNoLine}[1]{\HeadAux{\global\let\HeadLine=N#1}}%
    \noindent
    \begin{table*}[]
    \footnotesize
    \begin{tabular}{%
      >{\bfseries}lc|
      *{5}{c|}c>{\quad}c|
      *{2}{c|}c>{\quad}c
    }%
      &
      \head{Profile Alignment} &
      \head{Emotion} &
      \head{Conversation / Content} &
      \head{Social Awareness} &
      \head{Decisions / Reasoning} &
      \head{Opinion / Attitude}
      &
      &
      \head{Network Propagation} &
      \head{Network Structure} &
      \head{Social Dynamics} 
      &
      \\
      \sbox0{S}%
      \rule{0pt}{\dimexpr\ht0 + 2ex\relax}%
      Generative Agents \cite{park2023generative} & \greenbullet &&
        & & & &&
      \greenbullet & \greenbullet & 
      \\\hline
      WarAgent \cite{hua2023war} & \greenbullet &&
      & & & &&
       &  \greenbullet &
      \\\hline
      Social Simulacra \cite{park2022social} & && \greenbullet
        & & & &&
       &  & 
      \\\hline
      S3 \cite{gao2023s} & & \greenbullet & \greenbullet & & \greenbullet & \greenbullet & & \greenbullet & &
      \\\hline
      De Marzo et al. \cite{de2023emergence} & & & & & & & & & \greenbullet &
      \\\hline
      Humanoid Agents \cite{wang2023humanoid} & & \greenbullet & \greenbullet & & & \greenbullet & & & &
      \\\hline
      Lyfe Agents \cite{kaiya2023lyfe} & & & & & \greenbullet & & & & &
      \\\hline
      Zhang et al. \cite{zhang2023exploring} & & & & & & & & & & \greenbullet
      \\\hline
      AgentVerse \cite{chen2023agentverse} & & & & & & & & & & \greenbullet
      \\\hline
      Williams et al. \cite{williams2023epidemic} & & & & & \greenbullet & & & & &
      \\\hline
      Project Sid \cite{al2024project} & \greenbullet & & & \greenbullet & \greenbullet & & & \greenbullet & &
      \\\hline
      Li et al. \cite{li2023theory} & & & & \greenbullet & & & & & &
      \\\hline 
      Li et al. \cite{li2024large} & & & & & & & & \greenbullet & &
      \\\hline
      SpeechAgents \cite{zhang2024speechagents} & & & \greenbullet & & & & & & &
      \\\hline
      FPS \cite{liu2024skepticism} & & & & & & & & \greenbullet & & 
      \\\hline
      SOTOPIA \cite{zhou2023sotopia} & & & & \greenbullet & & & & & &
      \\\hline
      Zhang et al. \cite{zhang2024self} & & & \greenbullet & & & & & & &
      \\\hline 
      MetaAgents \cite{li2023metaagents} & \greenbullet & & & & & & & & &
      \\\hline
      Xie et al. \cite{xie2024can} & & & & \greenbullet & & & & & &
      \\\hline
      CRSEC \cite{ren2024emergence} & & & & \greenbullet & & & & \greenbullet & &
      \\\hline
      He et al. \cite{he2023homophily} & & & & & & & & & \greenbullet &
      \\\hline
      Wu et al. \cite{wu2024shall} & & & & & \greenbullet  & & & & & 
      \\\hline
      Digital Representatives \cite{jarrett2023language} & \greenbullet & & & & & & & & &
      \\\hline
      Affordable Generative Agents \cite{yu2024affordable} & \greenbullet & & \greenbullet & & & & & & \greenbullet &
      \\\hline
      Chuang et al. \cite{chuang2024wisdom} & & & & & & & & & & \greenbullet
      \\\hline 
      FUSE \cite{liu2024tiny} & & & & & & & & \greenbullet & &
      \\\hline
      HiSim \cite{mou2024unveiling} & & & \greenbullet & & & & & & & \greenbullet
      \\\hline
      OASIS \cite{yang2024oasis} & & & & & & & & \greenbullet & & \greenbullet
      \\\hline
      Sreedhar \& Chilton \cite{sreedhar2024simulating} & & & & & \greenbullet & & & & &
      \\\hline
      LMAgent \cite{liu2024lmagentlargescalemultimodalagents} & \greenbullet & & \greenbullet & & \greenbullet & & & & &
      \\\hline
      Gu et al. \cite{gu2025largelanguagemodeldriven} &  & &  \greenbullet & & & & & & & \greenbullet
      \\\hline
      Orlando et al. \cite{orlando2025generativeagentbasedmodelingreplicate} &  & &  & & & & & & & \greenbullet
      \\\hline
      Wang et al. \cite{wang2025user} & \greenbullet & &  & & & & & & & \greenbullet
      \\\hline
      Ferraro et al. \cite{Ferraro2025155} & & & \greenbullet  & & & & & & & \greenbullet
      \\\hline
      Zheng et al. \cite{Zheng202563} & & &  & & & & & & & \greenbullet
      \\\hline
      Total & 8 & 2 & 10 & 5 & 7 & 2 & & 8 & 5 & 10
      \\[.5ex]
      \multicolumn{2}{c}{} &
      \multicolumn{4}{c}{\bfseries Individual} &&&
      \multicolumn{2}{c}{\bfseries Group} &
      \\
      
    \end{tabular}%
    \caption{Classification of the reproduced social phenomena for the 35 papers}
    \label{tab:rq1}
    \end{table*}
    \kern19.5mm % manually with the help of the next \vrule
    % \vrule height 50mm
  \endgroup

==> tables/RQ2.tex <==
\begingroup
    \renewcommand*{\arraystretch}{1.5}%
    \definecolor{tabred}{RGB}{230,36,0}%
    \definecolor{tabgreen}{RGB}{0,116,21}%
    \definecolor{taborange}{RGB}{255,124,0}%
    \definecolor{tabbrown}{RGB}{171,70,0}%
    \definecolor{tabyellow}{RGB}{255,253,169}%
    \newcommand*{\redtriangle}{\textcolor{tabred}{\ding{115}}}%
    \newcommand*{\greenbullet}{\textcolor{tabgreen}{\ding{108}}}%
    \newcommand*{\orangebullet}{\textcolor{taborange}{\ding{108}}}%
    \newcommand*{\orangecirc}{\textcolor{taborange}{\ding{109}}}%
    \newcommand*{\headformat}[1]{{\footnotesize\bfseries#1}}%
    \newcommand*{\vcorr}{%
      \vadjust{\vspace{-\dp\csname @arstrutbox\endcsname}}%
      \global\let\vcorr\relax
    }%
    \newcommand*{\HeadAux}[1]{%
      \multicolumn{1}{@{}r@{}}{%
        \vcorr
        \sbox0{\headformat{\strut #1}}%
        \sbox2{\headformat{Complex Data Movement}}%
        \sbox4{\kern\tabcolsep\redtriangle\kern\tabcolsep}%
        \sbox6{\rotatebox{45}{\rule{0pt}{\dimexpr\ht0+\dp0\relax}}}%
        \sbox0{\raisebox{.5\dimexpr\dp0-\ht0\relax}[0pt][0pt]{\unhcopy0}}%
        \kern.75\wd4 %
        \rlap{%
          \raisebox{.25\wd4}{\rotatebox{45}{\unhcopy0}}%
        }%
        \kern.25\wd4 %
        \ifx\HeadLine Y%
        \showthe\dimen0 % Debugging: Check the computed width

          \dimen0=\dimexpr\wd2+.5\wd4\relax
          \rlap{\rotatebox{45}{\hbox{\vrule \vrule width 3cm height .4pt}}}%
        \fi
      }%
    }%
    \newcommand*{\head}[1]{\HeadAux{\global\let\HeadLine=Y#1}}%
    \newcommand*{\headNoLine}[1]{\HeadAux{\global\let\HeadLine=N#1}}%
    \noindent
    \begin{table*}[]
    \footnotesize
    \begin{tabular}{%
      >{\bfseries}lc|
      *{2}{c|}c>{\quad}c|
      *{2}{c|}c>{\quad}c
    }%
      &
      \head{Human(-like) Judgment} &
      \head{Social Patterns} &
      \head{Other Models} &
       &
      \head{Human Generated} &
      \head{Internal Consistency} &
      \head{Other Models} &
      &

      \\
      \sbox0{S}%
      \rule{0pt}{\dimexpr\ht0 + 2ex\relax}%
      Generative Agents \cite{park2023generative} & \greenbullet & \orangebullet
       &  & & & &  &
      \\\hline
      WarAgent \cite{hua2023war} & \greenbullet &
      & & & \greenbullet & \orangebullet & &
      \\\hline
      Social Simulacra \cite{park2022social} & \greenbullet &
      &  & & \orangebullet &&&
      \\\hline
      S3 \cite{gao2023s} & & & && \greenbullet &  & 
      \\\hline
      De Marzo et al. \cite{de2023emergence} & & \greenbullet & & & & \orangebullet & &  \\\hline
      Humanoid Agents \cite{wang2023humanoid} & & & && \greenbullet &  & \\\hline
      Lyfe Agents \cite{kaiya2023lyfe} & & \greenbullet & & & & & & \\\hline
      Zhang et al. \cite{zhang2023exploring} & & \greenbullet & & & & & & \\\hline
      AgentVerse \cite{chen2023agentverse} & & \greenbullet & & & & & & \\\hline
      Williams et al. \cite{williams2023epidemic} & & \greenbullet & & & & & & \\\hline
      Project Sid \cite{al2024project} & & \greenbullet & & & & & & \\\hline
      Li et al. \cite{li2023theory} & \greenbullet & \orangebullet & & & & & & & \\\hline
      Li et al. \cite{li2024large} & & \greenbullet & & & & & & \\\hline
      SpeechAgents \cite{zhang2024speechagents} & \greenbullet & & & & & & \orangebullet & \\\hline
      FPS \cite{liu2024skepticism} & & \greenbullet & & & & & &\\\hline
      SOTOPIA \cite{zhou2023sotopia} & \greenbullet & & && \orangebullet & & & \\\hline
      Zhang et al. \cite{zhang2024self} & \greenbullet & & && \greenbullet & & & \\\hline
      MetaAgents \cite{li2023metaagents} & \greenbullet & & & & & & & \\\hline
      Xie et al. \cite{xie2024can} & \greenbullet & & & && & & \\\hline
      CRSEC \cite{ren2024emergence} & \greenbullet & \orangebullet & &&  & & & & \\\hline
      He et al. \cite{he2023homophily} & & \orangebullet & & & & \greenbullet & &  \\\hline
      Wu et al. \cite{wu2024shall} & & \greenbullet & & & \orangebullet & & & \\\hline
      Digital Representatives \cite{jarrett2023language} & \orangebullet & & & & \greenbullet & & & \\\hline
      Affordable Generative Agents \cite{yu2024affordable} & \greenbullet & & \greenbullet & & & & \orangebullet & & \\\hline
      Chuang et al. \cite{chuang2024wisdom} & & & & & \greenbullet & & & \\\hline
      FUSE \cite{liu2024tiny} & & \greenbullet & & & & & & \\\hline
      HiSim \cite{mou2024unveiling} & & \orangebullet & & & \greenbullet & & \greenbullet & \\\hline
      OASIS \cite{yang2024oasis} & & \orangebullet & & & \greenbullet & & & \\\hline
      Sreedhar \& Chilton \cite{sreedhar2024simulating}  & & & & & \greenbullet & \orangebullet & & 
      \\\hline
      LMAgent \cite{liu2024lmagentlargescalemultimodalagents}  & \greenbullet & & \orangebullet & & \greenbullet & & & 
      \\\hline
      Gu et al. \cite{gu2025largelanguagemodeldriven}  & & & \orangebullet & & \greenbullet & & & 
      \\\hline
      Orlando et al. \cite{orlando2025generativeagentbasedmodelingreplicate}  & & \greenbullet &  & &  & & & 
      \\\hline
      Wang et al. \cite{wang2025user}  & \orangebullet & \greenbullet & \orangebullet & & \orangebullet & & & 
      \\\hline
      Ferraro et al. \cite{orlando2025generativeagentbasedmodelingreplicate}  & & \greenbullet &  & & \greenbullet & & & 
      \\\hline
      Zheng et al. \cite{Zheng202563}  & & \greenbullet &  & &  & & & 
      \\\hline
      Total (main technique) & 12 & 14  & 1 && 12 & 1 & 1
      \\\hline
      Total (secondary technique) & 2 & 6 & 3 & & 4 & 3 & 2
      \\[.5ex]
      \multicolumn{1}{c}{} &
      \multicolumn{3}{c}{\bfseries Subjective} &&
      \multicolumn{4}{c}{\bfseries Objective} &

      
    \end{tabular}%
    \caption{Classification of the validation techniques for the 35 papers.}
    \label{tab:rq2}
    \end{table*}
    \kern19.5mm % manually with the help of the next \vrule
    % \vrule height 50mm
  \endgroup

==> tables/RQ3.tex <==
\begingroup
    \renewcommand*{\arraystretch}{1.5}%
    \definecolor{tabred}{RGB}{230,36,0}%
    \definecolor{tabgreen}{RGB}{0,116,21}%
    \definecolor{taborange}{RGB}{255,124,0}%
    \definecolor{tabbrown}{RGB}{171,70,0}%
    \definecolor{tabyellow}{RGB}{255,253,169}%
    \definecolor{tabblue}{RGB}{93, 103, 245}
    \newcommand*{\redtriangle}{\textcolor{tabred}{\ding{115}}}%
    \newcommand*{\bluesquare}{\textcolor{tabblue}{\ding{110}}}%
    \newcommand*{\greenbullet}{\textcolor{tabgreen}{\ding{108}}}%
    \newcommand*{\orangebullet}{\textcolor{taborange}{\ding{108}}}%
    \newcommand*{\orangecirc}{\textcolor{taborange}{\ding{109}}}%
    \newcommand*{\headformat}[1]{{\small#1}}%
    \newcommand*{\vcorr}{%
      \vadjust{\vspace{-\dp\csname @arstrutbox\endcsname}}%
      \global\let\vcorr\relax
    }%
    \newcommand*{\HeadAux}[1]{%
      \multicolumn{1}{@{}r@{}}{%
        \vcorr
        \sbox0{\headformat{\strut #1}}%
        \sbox2{\headformat{Complex Data Movement}}%
        \sbox4{\kern\tabcolsep\redtriangle\kern\tabcolsep}%
        \sbox6{\rotatebox{45}{\rule{0pt}{\dimexpr\ht0+\dp0\relax}}}%
        \sbox0{\raisebox{.5\dimexpr\dp0-\ht0\relax}[0pt][0pt]{\unhcopy0}}%
        \kern.75\wd4 %
        \rlap{%
          \raisebox{.25\wd4}{\rotatebox{45}{\unhcopy0}}%
        }%
        \kern.25\wd4 %
        \ifx\HeadLine Y%
          \dimen0=\dimexpr\wd2+.5\wd4\relax
          \rlap{\rotatebox{45}{\hbox{\vrule width\dimen0 height .4pt}}}%
        \fi
      }%
    }%
    \newcommand*{\head}[1]{\HeadAux{\global\let\HeadLine=Y#1}}%
    \newcommand*{\headNoLine}[1]{\HeadAux{\global\let\HeadLine=N#1}}%
    \noindent
    \begin{table*}[]
    \begin{tabular}{%
      >{\bfseries}lc|
      *{4}{c|}c|>{\quad}c
    }%
      &
      \head{Complexity of the Real World} &
      \head{Lack of data / framework / truth} &
      \head{Lack of determinism} &
      \head{Bias} &
      \head{Hallucinations} &
      \head{Scalability} &

      \\
      \sbox0{S}%
      \rule{0pt}{\dimexpr\ht0 + 2ex\relax}%
      Generative Agents \cite{park2023generative} & & \bluesquare & & \bluesquare & \bluesquare & \bluesquare & 
      \\\hline
      WarAgent \cite{hua2023war} & \greenbullet & & & \greenbullet & \greenbullet & 
      \\\hline
      Social Simulacra \cite{park2022social} & \greenbullet & & & \greenbullet & \bluesquare & \bluesquare
      \\\hline
      S3 \cite{gao2023s} & \bluesquare & & & & & \bluesquare
      \\\hline
      De Marzo et al. \cite{de2023emergence} & & \bluesquare & & & \greenbullet &   \\\hline
      Humanoid Agents \cite{wang2023humanoid} & \bluesquare & & & & & \\\hline
      Lyfe Agents \cite{kaiya2023lyfe} & & \bluesquare & & & & \greenbullet  \\\hline
      Zhang et al. \cite{zhang2023exploring} & \bluesquare & & & \bluesquare & \bluesquare &  \\\hline
      AgentVerse \cite{chen2023agentverse} & & \bluesquare & & & & 
      \\\hline
      Williams et al. \cite{williams2023epidemic} & \greenbullet & \bluesquare & &\greenbullet & \bluesquare &  \\\hline
      Project Sid \cite{al2024project} & & \greenbullet & & \bluesquare & \greenbullet &   \\\hline
      Li et al. \cite{li2023theory} & \greenbullet & & & \bluesquare & & \bluesquare  \\\hline
      Li et al. \cite{li2024large} & & &  & \greenbullet & &  \\\hline
      SpeechAgents \cite{zhang2024speechagents} & &  & & & &  \\\hline
      FPS \cite{liu2024skepticism} & \greenbullet & & & & &  \\\hline
      SOTOPIA \cite{zhou2023sotopia} & \bluesquare &  &  & \bluesquare & \bluesquare & \bluesquare  \\\hline
      Zhang et al. \cite{zhang2024self} & & & & \bluesquare & \bluesquare & \greenbullet  \\\hline
      MetaAgents \cite{li2023metaagents} & \bluesquare & \greenbullet & & & \bluesquare & \bluesquare  \\\hline
      Xie et al. \cite{xie2024can} & \bluesquare & & & \bluesquare & & \\\hline
      CRSEC \cite{ren2024emergence} & & & & \bluesquare & \greenbullet & \bluesquare \\\hline
      He et al. \cite{he2023homophily} & \bluesquare & \bluesquare & \bluesquare & \bluesquare & &  \\\hline
      Wu et al. \cite{wu2024shall} & & \bluesquare & & \greenbullet & & \bluesquare & \\\hline
      Digital Representatives \cite{jarrett2023language} & & & & \bluesquare & & \\\hline
      Affordable Generative Agents \cite{yu2024affordable} & & \bluesquare & \greenbullet &  & \bluesquare & \greenbullet  \\\hline
      Chuang et al. \cite{chuang2024wisdom} & & \greenbullet & & \bluesquare & \bluesquare &  \\\hline
      FUSE \cite{liu2024tiny} & & \greenbullet & & & &   \\\hline
      HiSim \cite{mou2024unveiling} & \greenbullet &  & \greenbullet & \bluesquare & \bluesquare & \greenbullet   \\\hline
      OASIS \cite{yang2024oasis} & \greenbullet &  &  & \bluesquare & & \greenbullet  \\\hline
      Sreedhar \& Chilton \cite{sreedhar2024simulating}  & \greenbullet &  &  & \greenbullet & \bluesquare & \bluesquare  
      \\[.5ex]
      

      
    \end{tabular}%
    \caption{Classification of the challenge awareness for the 29 papers. Blue squares indicate the mention of a challenge, green bullets mean that the paper additionally implemented measures to mitigate the challenge or explained why the challenge is not applicable or not a problem.}
    \label{tab:rq3}
    \end{table*}
    \kern19.5mm % manually with the help of the next \vrule
    % \vrule height 50mm
  \endgroup
